Online Planning in POMDPs with State-Requests

In key real-world problems, full state information is sometimes available but only at a high cost, like activating precise yet energy-intensive sensors or consulting humans, thereby compelling the agent to operate under partial observability. For this scenario, we propose AEMS-SR (Anytime Error Minimization Search with State Requests), a principled online planning algorithm tailored for POMDPs with state requests. By representing the search space as a graph instead of a tree, AEMS-SR avoids the exponential growth of the search space originating from state requests. Theoretical analysis demonstrates AEMS-SR's $\varepsilon$-optimality, ensuring solution quality, while empirical evaluations illustrate its effectiveness compared with AEMS and POMCP, two SOTA online planning algorithms. AEMS-SR enables efficient planning in domains characterized by partial observability and costly state requests offering practical benefits across various applications.

==> algo_3.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{GWalk: computing $\cumProbDirect$ and $\cumProbDirect_{\rootBelief}$}\label{alg:gwalk}
\SetKwInOut{Input}{input}
\Input{belief $\belief$, visitedStates $\mathcal{V}$, stateMatrix $M$, $\bar{p}$, fringeNodes $\hat{\fringe}$, Graph $\graph$, root belief $\rootBelief$}
\tcc{Recursive algorithm, modifies inputs in place. }
\If{$\belief \in \fringe\fun{\graph}$}{
    $\hat{\fringe} = \hat{\fringe} \cup \{\belief\}$\;
}
\ElseIf{$\pi(\belief) = \request$}{
    \For{$\state \in \support\fun{\belief}$}{
        \If{$\origin\fun{\belief} = \rootBelief$}{
            $\bar{p}$[$\state$] += $\belief[\state] * \cumProbDirect(\origin(\belief), \belief$)\;
        }
        \Else{
            $M_{\origin(\belief), \state} += \belief[\state] * \cumProbDirect(\origin(\belief), \belief$)\;
        }
        \If{$\state \notin \mathcal{V}$}{
            $\mathcal{V} = \mathcal{V} \cup \{\state\}$\;
            \For{$\observation \in \observationfn(\state, \pi(\state))$}{
                \texttt{GWalk}($\tau\fun{\state, \pi(\state), \observation}, \mathcal{V}, M, \bar{p}, \hat{\fringe}$)\;
            }
        }
    }
}
\Else{
    \For{$\observation \in \observationfn(\belief, \pi(\belief))$}{
        \texttt{GWalk}($\tau\fun{\belief, \pi(\belief), \observation}, \mathcal{V}, M, \bar{p}, \hat{\fringe}$)\;
    }
}
\end{algorithm}


==> pbvi_sr.tex <==
\section{Offline planning: PBVI-SR}



The extension of PBVI to the POMDP-SR framework, denoted as PBVI-SR, provides an intuitive adaptation that maintains the core structure, and limitations, of PBVI type algorithms. 
Although our main focus is on online methods, which offer better scalability, we illustrate here for completeness how classical offline methods of the PBVI family can be extended to POMDP-SR.

\begin{figure}[h]
    \centering
    \includegraphics[width=.4\linewidth]{img/pbvi_sr.pdf}
    \caption{PBVI-SR: modifications of the original algorithm are in red.}
    \label{fig:pbvi_sr}
\end{figure}
As previously stated, PBVI approximates the belief space using a finite set of representative points and conducts iterative backward induction from the final time-step.
In the following we introduce two critical modifications to the application of PBVI on the original POMDP to avoid any unnecessary computation and without modifying the spirit of the algorithm.
First, the belief set is enriched with the corner beliefs. This ensures that no additional approximation are needed when requesting the state.
Second, during the construction of $\alpha$-vectors for time-step $t$, an additional alpha vector is introduced at the end. This extra alpha vector represents the expected value of occupying a state $\state_i$, which can be easily computed based on the other alpha vectors of time-step $t$, minus the cost $c$. Figure \ref{fig:pbvi_sr} shows how the additional $\alpha$-vector $\alpha_c$ is constructed in a 2 state POMDP.  
During execution, when the agent's belief aligns with this supplementary alpha vector, it triggers a state request. Subsequently, the belief is replaced with the corresponding corner belief, enabling the selection of the environmental action. This adaptive mechanism empowers the agent to make informed decisions regarding when to request the state, seamlessly integrating this capability within the PBVI framework.

It is important to note that while PBVI-SR offers an initial offline solution for POMDP-SR scenarios, it shares common limitations with offline methods. Specifically, PBVI-SR pre-computes a solution for the entire belief space, restricting its applicability to larger problems. Additionally, while the solution quality improves with a larger belief set, it also increases the computational complexity of the algorithm.

